Comprehensive Dataset of Face Manipulations for Development and Evaluation of Forensic Tools

Digital media (e.g., photographs, video) can be easily created, edited, and shared. Tools for editing digital media are capable of doing so while also maintaining a high degree of photo-realism. While many types of edits to digital media are generally benign, others can also be applied for malicious purposes. State-of-the-art face editing tools and software can, for example, artificially make a person appear to be smiling at an inopportune time, or depict authority figures as frail and tired in order to discredit individuals. Given the increasing ease of editing digital media and the potential risks from misuse, a substantial amount of effort has gone into media forensics. To this end, we created a challenge dataset of edited facial images to assist the research community in developing novel approaches to address and classify the authenticity of digital media. Our dataset includes edits applied to controlled, portrait-style frontal face images and full-scene in-the-wild images that may include multiple (i.e., more than one) face per image. The goals of our dataset is to address the following challenge questions: (1) Can we determine the authenticity of a given image (edit detection)? (2) If an image has been edited, can we \textit{localize} the edit region? (3) If an image has been edited, can we deduce (classify) what edit type was performed? The majority of research in image forensics generally attempts to answer item (1), detection. To the best of our knowledge, there are no formal datasets specifically curated to evaluate items (2) and (3), localization and classification, respectively. Our hope is that our prepared evaluation protocol will assist researchers in improving the state-of-the-art in image forensics as they pertain to these challenges.

==> related.tex <==
\section{Related Work}

The state-of-the-art in image editing can appear realistic enough such that it is extremely difficult, if not impossible for a human examiner to identify computer-generated content. The faithfulness of media presents a profound set of problems, including societal (public trust of information and dis-information campaigns) and for national security (identity management). Consequently, as image and media editing software has become more realistic, readily available, and user-friendly, forensic analysis and forgery detection is an increasingly more important area of research. 


\subsection{Detecting Manipulations in Face Images}
\begin{itemize}
    \item Early approaches for detecting manipulated images relied on image processing techniques such as  
    \item modeling photo-response nonuniformity (PRNU)  \cite{chen2008determining}\cite{chierchia2010influence}\cite{rathgeb2020prnu}
    \item Other research investigates approaches to detect morphed (blended) faces \cite{raja2017transferable}\cite{scherhag2018detecting}\cite{neubert2017face} to defend against the possibility of multi-face authentication from a single token \cite{6996240}.
    \item With the advent of deep learning, many researchers have proposed and developed convolutional neural network models to detect face swapping and face reenactment \cite{zhou2017two}\cite{rossler2018faceforensics}\cite{rossler2019faceforensics++}. 
    
    \item Wang et al. attempt to train a binary classifier to detect face shape editing from Adobe Photoshop \cite{wang2019detecting}.
\end{itemize}

\subsection{Datasets}
\begin{itemize}
    \item The literature is generally lacking standardized datasets for detecting and classifying manipulations in face images.
    \item Many researchers create their own datasets and perform subsequent test and evaluation on that data \cite{wang2019detecting}. In general, this raises concerns regarding the ability of proposed approaches to generalize to unseen data or data that is out-of-distribution.
\end{itemize}
